Transfer Learning for Latent Variable Network Models

We study transfer learning for estimation in latent variable network models. In our setting, the conditional edge probability matrices given the latent variables are represented by $P$ for the source and $Q$ for the target. We wish to estimate $Q$ given two kinds of data: (1) edge data from a subgraph induced by an $o(1)$ fraction of the nodes of $Q$, and (2) edge data from all of $P$. If the source $P$ has no relation to the target $Q$, the estimation error must be $\Omega(1)$. However, we show that if the latent variables are shared, then vanishing error is possible. We give an efficient algorithm that utilizes the ordering of a suitably defined graph distance. Our algorithm achieves $o(1)$ error and does not assume a parametric form on the source or target networks. Next, for the specific case of Stochastic Block Models we prove a minimax lower bound and show that a simple algorithm achieves this rate. Finally, we empirically demonstrate our algorithm's use on real-world and simulated graph transfer problems.

==> acknowledgments.tex <==
\begin{ack}
We thank...
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

==> algorithm-rank2.tex <==
% !TEX root = ./neurips_2024.tex

\section{Estimating Latent Variable Models with Rankings}
%\label{sec:rankings}
In this section we present a computationally efficient transfer learning algorithm for latent variable models. Algorithm~\ref{alg:q-averaging-row-wise} learns the local structure of $P$ based on graph distances (Definition~\ref{defn:graph-distance}). For each node $i$ of $P$, it ranks the nodes in $S$ with respect to the graph distance $d_P(i, \cdot)$. For most nodes $i, j \in [n]$, none of the edges incident to $i$ or $j$ are observed in $Q$. Therefore, we estimate $\hat Q_{ij}$ by using the edge information about nodes $r, s \in S$ such that $d_P(i, r)$ and $d_P(j, s)$ are small. 




==> checklist.tex <==
% !TEX root = ./neurips_2024.tex

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss our main contributions in the abstract and introduction, and then develop them in the main body of the paper. Specifically, we point out Algorithm~\ref{alg:q-averaging-row-wise} and Algorithm~\ref{alg:q-perfect-clustering}, the upper bounds from Theorem~\ref{thm:alg1error} and Proposition~\ref{prop:q-perfect-clustering}, and the lower bound Theorem~\ref{thrm:minimax-sbm}. Finally, Section~\ref{sec:experiments} shows experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitation of lacking a minimax lower bound for network estimation in $d$-dimensions after Theorem~\ref{thm:alg1error}, the need for a different graph distance for graphs with sparsity $O(\frac{\log n}{n})$ in the Conclusion, and adapting to multiple source distributions in the Conclusion. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give self-contained theoretical statements with definitions and assumptions in the main body, and full proofs for all claims in Appendix~\ref{appendix:proofs}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give experimental details in Section~\ref{sec:experiments}, and give further details on our exact data preparation methods in Appendix~\ref{appendix:experiment-details}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We submit our code as a supplementary zip file in accordance with the NeurIPS code and data submission guidelines. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our choices of source and target network, the network sizes and degrees, and the single hyperparameter (quantile cutoff) for Algorithm~\ref{alg:q-averaging-row-wise} in Section~\ref{sec:experiments}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experiment we run $50$ independent trials. We report $\pm 2$ standard deviations for the mean-squared error in Table~\ref{table:simul-results}, and $[1,99]$ percentile errors in Figure~\ref{fig:realworld}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

% \blue{}
\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As described in Appendix~\ref{appendix:experiment-details}, we run all experiments on a personal Linux machine with 378GB of CPU/RAM. The total compute time  across all results in the paper was less than $2$ hours.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} 
    %Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conform with the NeurIPS Code of Ethics with regards to potential harms caused by the research process, societal impact, and impact mitigation measures. Moreover, we have anonymized our code and manuscript. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper presents work whose goal is to advance the field of Machine Learning through foundational research. There are many possible societal consequences of our work, none which we feel must be specifically highlighted here.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release data or models that have a high risk for misuse. We use only publicly available data from the academic literature. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We credit the authors of the BiGG metabolic models dataset~\citep{bigg-models,norsigian2020bigg} and the \textsc{Email-EU} dataset \citep{snapnets,motifs-2017}. Both datasets are publicly released for academic research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release new assets. See Appendix~\ref{appendix:experiment-details} for the exact details regarding our use of existing datasets and assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not perform any crowdsourcing or research on human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not perform any research on living subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}
\end{enumerate}


==> proposed-work.tex <==
% !TEX root = ./neurips_2024.tex

%\subsection{Proposed Work}
%\label{sec:proposed}

{\bf Transfer learning on networks.} We wish to estimate the target network $Q$. However, we only observe $f_Q$ on $\binom{n_Q}{2}$ pairs of nodes, for a uniformly random subset of variables $S \subset \{1, 2, \dots, n\}$. We assume $S$ is vanishingly small, so $\abs{S} := n_Q = o(n)$.
% estimate $f_Q$solve 
% Problem~\ref{prob:network-estimation} for 

Absent additional information, we cannot hope to achieve $o(1)$ mean-squared error. To see this, suppose $f_Q$ is a stochastic block model with $2$ communities of equal size. For a node $i \not \in S$, no edges incident to $i$ are observed, so its community cannot be learned. Since $n_Q \ll n$, we will attain $\Omega(1)$ error overall. To attain error $o(1)$, we hope to leverage transfer learning from a source $P$ if available. In fact, we give an efficient algorithm to achieve $o(1)$ error, informally stated below.
% Formally stated in Theorem~\ref{thm:alg1error}.
%Theorem~\ref{thm:erroralg1}:
\begin{theorem}[Theorem~\ref{thm:alg1error}, Informal]
There exists an efficient algorithm such that, if given source data $A_P \in \{0,1\}^{n \times n}$ and target data $A_Q \in \{0,1\}^{n_Q \times n_Q}$ coming from an {\em appropriate} pair $(f_P, f_Q)$ of latent variable models, outputs $\hat Q \in \RR^{n \times n}$ such that: 
\[
\PP\bigg[\frac{1}{n^2} \norm Q - \hat Q \norm_F^2 \leq o(1)\bigg] \geq 1 - o(1).
\]
\label{thrm:main-informal}
\end{theorem}
There must be a relationship between P and Q for them to be an {\em appropriate} pair for transfer learning. We formalize this relationship below.
% The kinds of additional data about $f_Q$, if any, will depend on the application. Different kinds of information enable different transfer learning algorithms. We consider a setting where both isolating nodes and testing edges are hard. Therefore, one might only be able to gather a small subset $S \subset [n_P]$ of nodes and then test the edges within $S$. %For example, metabolic networks model the chemical interactions related to release and utilization of energy within an organism \cite{Christensen2000}. Determining metabolic interactions {\em in vivo} requires metabolite balancing and labeling experiments, so only the edges whose endpoints are {\em both} incident to the experimentally chosen metabolites are observed \cite{Christensen2000}. For a non-model organism $Q$, the experimentally tested metabolites may be a small fraction of all metabolites believed to affect metabolism. However, more interaction data might be available for a model organism $P$, motivating transfer learning for biological networks \cite{kshirsagar2015combine}. 
% We formalize the general transfer learning problem as follows. 

% \begin{problem}[Transfer Learning for Target Network Estimation]
% For $S \subset [n]$ of size $n_Q$, 

% Given network data $(A_{P;ij})_{1 \leq i, j \leq n_P}$ and $(A_{Q;ij})_{i, j \in S}$ according to Eq.~\eqref{eq:latent-model} for source function $f_P$ and target function $f_Q$ respectively, where $S \subset [n_P]$ has size $n_Q = o(1)$, construct estimates $\{\hat f_Q(\bx_i, \bx_j): 1 \leq i, j \leq n_P\}$ so as to minimize mean-squared error: 
% \begin{align*}
% \mathrm{MSE}(\hat f_Q, f_Q) := \frac{1}{n_P^2} \sum\limits_{1 \leq i, j \leq n_P} (\hat f_Q(\bx_i, \bx_j) - f_Q(\bx_i, \bx_j))^2
% \end{align*}
% \label{prob:transfer-learning}
% \end{problem}

{\bf Relationship between source and target.} 
%For transfer learning to be useful, we need some relation between $f_P, f_Q$. To see this, consider the same example as above where $f_Q$ is a stochastic block model, and $f_P$ does not depend on the latent variables at all. For example, if $f_P \equiv \frac{1}{2}$ is Erdos-Renyi, then we will still achieve $\Omega(1)$ error.
%What kind of assumption can make transfer learning possible? 
It is natural to consider pairs $(f_P, f_Q)$ such that for all $\bx, \by \in \mathcal{X}$, the difference $(f_P(\bx, \by) - f_Q(\bx, \by))$ is small. For example, \cite{cai-pu-2024} study transfer learning for nonparametric regression when $f_P - f_Q$ is close to a polynomial in $\bx, \by$.
% consider transfer in nonparametric regression, where%  give guarantees for a local polynomial regression algorithm where we are given $(x_i,y_i)$ pairs of the form $y_i=f(x_i)+\epsilon_i$ in the source domain and  $y'_i=f'(x'_i)+\epsilo%n'_i$ in the target domain. The goal is to do transfer when $f-f'$ is $\epsilon$ close to a polynomial (\rd what kind of polynomial\bk) in $L_1$ norm. 
% However, in our setting the latent variables are unseen. 
But, requiring $f_P-f_Q$ to be pointwise small does not capture a broad class of pairs in the network setting. For example, if $f_P = \alpha f_Q$. Then $f_P - f_Q = (\alpha-1)f_Q$ can be far from all polynomials if $f_Q$ is, e.g. a \holder-smooth graphon.\footnote{In fact, \cite{cai-pu-2024} highlight this exact setting as a direction for future work.} However, under the network model, this means $A_P$ and $A_Q$ are stochastically identical modulo one being $\alpha$ times denser than the other. 
%So transfer should in fact be easy in this setting, i.e. if I know $P(A_P(i,j)=1|\bx_i,\bx_j)$, then corrsponding $Q$ probability is $1/\alpha$ times  the  former. 
We will therefore consider pairs $(f_P,f_Q)$ that are close in some measure of local graph structure. With that in mind, we use a graph distance  introduced in~\cite{mcs21} for a different inference problem.
\newcommand{\be}{\bm{e}}
\begin{defn}[Graph Distance]\label{defn:graph-distance}
Let $P \in [0,1]^{n \times n}$ be the probability matrix of a graph. For $i, j \in [n]$ we will use the the graph distance between $i, j$, $i\neq j$ as: 
\[
d_P(i, j) := \norm (\be_i - \be_j)^T P^2 (I - \be_i \be_i^T - \be_j \be_j^T)\norm_2^2
\]
Where $\be_i, \be_j \in \RR^{n}$ are standard basis vectors. 
\end{defn}
Intuitively, this first computes the matrix $P^2$ of common neighbors, and then computes the distance between two rows of the same (ignoring the diagonal elements). 
We will require that $f_P, f_Q$ satisfy a local similarity condition on the relative rankings of nodes with respect to this graph distance. Since we only estimate the probability matrix of $Q$, the condition is on the latent variables $\bx_1, \dots, \bx_n$ of interest.  The hope is that the proximity in graph distance reflects the proximity in latent positions.
\begin{defn}[Rankings Assumption at quantile $h_n$]
Let $(P, Q)$ be a pair of graphs evaluated on $n$ latent positions. We say $(P, Q)$ satisfy the rankings assumption at quantile $h_{n} \leq 1$ if there exists constant $C > 0$ such that
for all $j \neq i$, if $j$ belongs to the bottom $h_n$-quantile of $d_P(i, \cdot)$, then $j$ belongs to the bottom $Ch_n$-quantile of $d_Q(i, \cdot)$. 
\label{defn:ranks}
\end{defn}
Note that the condition is for relative, not absolute graph distances.
%If e.g. $f_P = 10 f_Q$ then absolute graph distances $d_P(\cdot, \cdot)$ are much larger than $d_Q(\cdot, \cdot)$ but the relative rankings of nodes in graph distance are identical. 

To illustrate Definition~\ref{defn:ranks}, consider stochastic block models $f_P, f_Q$ with $k_P \geq k_Q$ communities respectively. If nodes $i, j$ are in the same communities then $P \be_i = P \be_j$, so $d_P(i, j) = 0$. We require that $j$ minimizes $d_Q(i, \cdot)$. This occurs if and only if $d_Q(i, j) = 0$. Hence if $i, j$ belong to the same community in $P$, they are in the same community in $Q$. Note that the converse is not necessary; we could have $Q$ with $1$ community and $P$ with arbitrarily many communities. 

% The general transfer learning problem is then as follows. 

% \begin{problem}[Transfer Learning - This Paper]
% Given network data $(A_{P;ij})_{1 \leq i, j \leq n_P}$ and $(A_{Q;ij})_{i, j \in S}$ according to Eq.~\eqref{eq:latent-model}, for $S \subset \{1, \dots, n_P\}$ of size $n_Q$ chosen uniformly at random, and source-target pair $(f_P, f_Q)$ satisfying Assumption~\ref{assumption:ranks} at quantile $h_n$, 
%  for source function $f_P$ and target function $f_Q$ respectively, where $S \subset [n_P]$ has size $n_Q = o(1)$, construct estimates $\{\hat f_Q(\bx_i, \bx_j): 1 \leq i, j \leq n_P\}$ so as to minimize mean-squared error: 
% \begin{align*}
% \mathrm{MSE}(\hat f_Q, f_Q) := \frac{1}{n_P^2} \sum\limits_{1 \leq i, j \leq n_P} (\hat f_Q(\bx_i, \bx_j) - f_Q(\bx_i, \bx_j))^2
% \end{align*}
% \label{prob:transfer-learning-ours}
% \end{problem}

%\paragraph{Our Contributions.}
With the relationship between 
the source and target defined by the rankings assumption, our contributions are as follows.

% we first provide a simple algorithm for Stochastic Block Models (SBM), when the latent positions are shared and can be estimated consistently. We obtain the minimax lower bound for this and show that our simple algorithm matches this. 

% However, in general, one does not know 
% which model the graphs are coming from. And even if one did, assuming that both target and source distributions are of the parametric form $f_P(\bx_i,\bx_j)=\bx_i^TD_P\bx_j$, and $f_Q(\bx_i,\bx_j)=\bx_i^TD_Q\bx_j$, where $D_P$ and $D_Q$ are different square symmetric matrices is restrictive. There has been a rising interest in goodness of fit tests in network models \rd(cite stuff)\bk. Our next algorithm does not assume any particular parametric form of $f_P$ or $f_Q$, rather it works under %the assumption that one can construct graph-based distances which can act like proxies for distances between the latent positions. 

%\blue{AJ: where to put this? However, in general, one does not know which model the graphs are coming from. Therefore, we give a more general algorithm that does not assume any parametric form of $f_P$ or $f_Q$. }

{\bf (1) Algorithm for Latent Variable Models.}
We provide an efficient Algorithm~\ref{alg:q-averaging-row-wise} for latent variable models with H{\"o}lder-smooth $f_P, f_Q$. The benefit of this algorithm is that it does not assume a  parametric form of $f_P$ and $f_Q$.  We prove a guarantee on its error in Theorem ~\ref{thm:alg1error}. 

{\bf (2) Minimax Rates.}  We prove a minimax lower bound for Stochastic Block Models (SBMs) in Theorem~\ref{thrm:minimax-sbm}. Moreover, we provide a simple Algorithm~\ref{alg:q-perfect-clustering} that attains the minimax rate for this class (Proposition~\ref{prop:q-perfect-clustering}). 

{\bf (3) Experimental Results on Real-World Data.} We test both of our algorithms on real-world metabolic networks and dynamic email networks, as well as synthetic data 
% (Section~\ref{sec:experiments}).

All proofs are deferred to the Appendix.
% \begin{enumerate}
% 	\item We prove a minimax lower bound for Stochastic Block Models (SBMs) in Theorem~\ref{thrm:minimax-sbm}. 
% 	\item We provide a simple Algorithm~\ref{alg:q-perfect-clustering} and prove that it attains the minimax rate (Proposition~\ref{prop:q-perfect-clustering}). 
% 	\item We provide an Algorithm~\ref{alg:q-averaging-row-wise} for general latent variable models with $f_P, f_Q$ Holder-smooth. Moreover, a provable guarantee (Theorem ~\ref{thrm:error-row-wise}).
% 	\item Experimental results for Algorithm~\ref{alg:q-averaging-row-wise} on real-world metabolic networks and dynamic email networks, as well as simulated networks (Section~\ref{sec:experiments}).
% \end{enumerate}




